A Role-Based Approach for Orchestrating Emergent Configurations in the Internet of Things

The Internet of Things (IoT) is envisioned as a global network of connected things enabling ubiquitous machine-to-machine (M2M) communication. With estimations of billions of sensors and devices to be connected in the coming years, the IoT has been advocated as having a great potential to impact the way we live, but also how we work. However, the connectivity aspect in itself only accounts for the underlying M2M infrastructure. In order to properly support engineering IoT systems and applications, it is key to orchestrate heterogeneous 'things' in a seamless, adaptive and dynamic manner, such that the system can exhibit a goal-directed behaviour and take appropriate actions. Yet, this form of interaction between things needs to take a user-centric approach and by no means elude the users' requirements. To this end, contextualisation is an important feature of the system, allowing it to infer user activities and prompt the user with relevant information and interactions even in the absence of intentional commands. In this work we propose a role-based model for emergent configurations of connected systems as a means to model, manage, and reason about IoT systems including the user's interaction with them. We put a special focus on integrating the user perspective in order to guide the emergent configurations such that systems goals are aligned with the users' intentions. We discuss related scientific and technical challenges and provide several uses cases outlining the concept of emergent configurations.

==> iot-platforms.tex <==
\subsection{Platform Interoperability}

While protocols such as MQTT provide a straightforward manner to ensure communication (message passing) between devices that are connected to the same platform, the same does not hold when one attempts to connect devices registered to different platforms. Moreover, it proves to be challenging to redirect sensor data streams to a platform other than the one where the respective sensor has been registered. This is often the case because the business model of the platform providers is to establish themselves as the IoT hub, paying little attention to platform interoperability issues. We hypothesize that  platforms designed with the specific goal of interfacing and bringing together data from different platforms will be instrumental in the coming years. The Crossbreed platform has been suggested as one such attempt to bridge this gap.


\item providing computational building blocks to ease manipulating, processing and fusing data stream before the data is stored to the DB

types of fees

protocols: mobile operators are expected to play an increasingly important role in IoT platforms with the coming of LTE for IoTprotocols, which are deemed to enable long range, low power, large scale sensor deployments, by connecting them directly to the existing BTS infrastructure.








The notion of commitments can be included as part of the larger context of normative MAS \cite{Boella2006}, where some form of regulations (e.g. externally imposed or mutually agreed) are enforced onto the agents' behavior. In addition, normative systems also provide the sanctions against violations of the enforced behavior, based on which agents can decide whether to comply with these norms or not. To this end, several normative languages have been proposed with varying degrees of complexity. For instance, a normative language based on deontic logic with deadline operators is introduced in \cite{Vazquez-Salceda2004}, relying on concepts such as  obligations, permissions and prohibitions. Similarly, in \cite{Oren2009}, the authors formalize an electronic contracting language, introducing clauses within contracts for the parties involved. We further refer the reader to \cite{Criado2011} for a comprehensive survey on normative MAS. Now, given that ECs imply temporary (often short-lived) cooperation between IoT devices with varying degrees of processing capabilities, we resort here to commitments as a simple and basic means of managing interaction.


@Article{Boella2006,
author="Boella, Guido
and van der Torre, Leendert
and Verhagen, Harko",
title="Introduction to normative multiagent systems",
journal="Computational {\&} Mathematical Organization Theory",
year="2006",
volume="12",
number="2",
pages="71--79"
}

@Inbook{Oren2009,
author="Oren, Nir
and Panagiotidi, Sofia
and V{\'a}zquez-Salceda, Javier
and Modgil, Sanjay
and Luck, Michael
and Miles, Simon",
editor="H{\"u}bner, Jomi Fred
and Matson, Eric
and Boissier, Olivier
and Dignum, Virginia",
title="Towards a Formalisation of Electronic Contracting Environments",
bookTitle="Coordination, Organizations, Institutions and Norms in Agent Systems IV : COIN 2008 International Workshops, COIN@AAMAS 2008, Estoril, Portugal, May 12, 2008. COIN@AAAI 2008, Chicago, USA, July 14, 2008. Revised Selected Papers",
year="2009",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="156--171",
}


@Inbook{Vazquez-Salceda2004,
author="V{\'a}zquez-Salceda, Javier
and Aldewereld, Huib
and Dignum, Frank",
editor="Lindemann, Gabriela
and Denzinger, J{\"o}rg
and Timm, Ingo J.
and Unland, Rainer",
title="Implementing Norms in Multiagent Systems",
bookTitle="Multiagent System Technologies: Second German Conference, MATES 2004, Erfurt, Germany, September 29-30, 2004. Proceedings",
year="2004",
publisher="Springer Berlin Heidelberg",
address="Berlin, Heidelberg",
pages="313--327"
}


@article{Criado2011,
 author = {Criado, N. and Argente, E. and Botti, V.},
 title = {Open Issues for Normative Multi-agent Systems},
 journal = {AI Commun.},
 issue_date = {August 2011},
 volume = {24},
 number = {3},
 month = aug,
 year = {2011},
 issn = {0921-7126},
 pages = {233--264},
 numpages = {32},
 acmid = {2350122},
 publisher = {IOS Press},
 address = {Amsterdam, The Netherlands, The Netherlands},
} 
